SynCode: LLM Generation with Grammar Augmentation

LLMs are widely used in complex AI applications. These applications underscore the need for LLM outputs to adhere to a specific format, for their integration with other components in the systems. Typically the format rules e.g., for data serialization formats such as JSON, YAML, or Code in Programming Language are expressed as context-free grammar (CFG). Due to the hallucinations and unreliability of LLMs, instructing LLMs to adhere to specified syntax becomes an increasingly important challenge. We present SynCode, a novel framework for efficient and general syntactical decoding with LLMs, to address this challenge. SynCode ensures soundness and completeness with respect to the CFG of a formal language, effectively retaining valid tokens while filtering out invalid ones. SynCode uses an offline-constructed, efficient lookup table, the DFA mask store, derived from the DFA of the language's grammar for efficient generation. SynCode seamlessly integrates with any language defined by CFG, as evidenced by experiments focusing on generating JSON, Python, and Go outputs. Our experiments evaluating the effectiveness of SynCode for JSON generation demonstrate that SynCode eliminates all syntax errors and significantly outperforms state-of-the-art baselines. Furthermore, our results underscore how SynCode significantly reduces 96.07% of syntax errors in generated Python and Go code, showcasing its substantial impact on enhancing syntactical precision in LLM generation. Our code is available at https://github.com/uiuc-focal-lab/syncode

==> algorithms/lookup_table.tex <==
\begin{wrapfigure}{R}{0.53\textwidth}
\vspace{-.34in}
\begin{minipage}{0.55\textwidth}

\begin{algorithm}[H]

\caption{Computing Lookup Table}
\label{alg:lookup}
%
\textbf{Inputs:} $\allterminals$: all terminals in the grammar, $\vocab$: vocabulary
\begin{algorithmic}[1]
\Function{compute\_lookup\_table}{$\allterminals$, $\vocab$}
\For{$\terminal \in \allterminals$}
\State $\dfa_{\terminal} \gets \text{ComputeDFA}(\terminal)$
\For{$q_{\terminal} \in Q_{\terminal}, t \in \vocab$}
% \State 
\EndFor
\EndFor
% \State $A_{j+1}, A_{j}, r \gets \text{Parse}(C_i)$
% \State $m \gets \Big(\bigcup_{\terminal \in A_j} L(\terminal, r)\Big) \cup \Big(\bigcup_{\terminal \in A_{j+1}} L(\terminal, \epsilon)\Big)$
\State \Return $m$
\end{algorithmic}
\end{algorithm}

\end{minipage}
\vspace{-0.2in}
\end{wrapfigure}

==> grammars/c_grammar.tex <==
\lstdefinestyle{myGrammarStyle}{
    basicstyle=\scriptsize\ttfamily, % Reduce font size
    commentstyle=\color{gray},
    keywordstyle=\color{blue},
    stringstyle=\color{orange},
    numbers=left, % Line numbers on left
    numberstyle=\tiny\color{gray}, % Line numbers styling
    breaklines=true, % Wrap long lines
    frame=single, % Frame around the code
    framesep=3pt, % Adjust frame separation
    xleftmargin=5pt, % Adjust left margin
    xrightmargin=5pt, % Adjust right margin
    backgroundcolor=\color{yellow!4}, % Background color
    tabsize=2, % Tab size
    captionpos=b, % Caption position bottom
    aboveskip=5pt, % Reduce space above the listing
    belowskip=5pt, % Reduce space below the listing
    linewidth=0.9\linewidth, % Set custom line width to less than text width
    escapeinside={(*@}{@*)}, % for escaping to LaTeX
}

\begin{lstlisting}[style=myGrammarStyle, caption=C Grammar]
start: declaration*

declaration: data_type NAME "(" parameter? ")" "{" statement* "}"

statement: data_type NAME "=" expression ";" 
            | NAME  "="  expression ";" 
            | NAME  "(" arg_list? ")" ";" 
            | "return"  expression ";" 
            | "while" "(" condition ")" "{" statement* "}" 
            | "for" "(" for_init ";"  condition ";"  for_update ")" "{" statement* "}" 
            | "if" "(" condition ")" "{" statement* "}" ("else" "{" statement* "}")? 
            | single_line_comment 
            | multi_line_comment

data_type: "int" | "float"  | "char" | "void"
NAME: /[a-zA-Z_][a-zA-Z_0-9]*/

parameter: data_type NAME

for_init: data_type NAME  "="  expression | NAME  "="  expression
for_update: NAME  "="  expression

condition: expression relation_operator expression
relation_operator: ("<=" | "<" | "==" | "!=" | ">=" | ">")

expression: term (("+" | "-") term)*
term: factor(("*" | "/") factor)*

factor: NAME | number | unary_term | func_call | paren_expression
unary_term: "-" factor
func_call: NAME "(" arg_list? ")"
paren_expression: "("  expression  ")"

arg_list: expression (","  expression)*

number: /[0-9]+/

single_line_comment: /\/\/([^\n])*\n/ "\n"
multi_line_comment: /\/\*(.|\n)*?\*\//

WS : /[ \t\n]+/
%ignore WS

\end{lstlisting}
\label{gram:c_grammar}


==> tables/main_eval_go.tex <==
% \begin{wraptable}{r}{.6\textwidth} 
\begin{table}[b]
    \tablesize
    \centering
    % \vspace{-0.15in}
    \caption{Effectiveness of \Tool{} in generating syntactic Go code}
    \begin{tabular}{@{}ll ccc@{}}
        \toprule
        Dataset & Architecture & \Baseline{} & \Tool{} & $\downarrow$ \\
        \hline
         & CodeGen-350M  & 573 & 49 & 91\% \\
        HumanEval & WizardCoder-1B  & 1031 & 50 & 95\% \\
        & Llama-7B  & 725 & 10 & 99\% \\
        \hline
        & CodeGen-350M  & 212 & 2 & 99\% \\
        MBXP & WizardCoder-1B  & 243 & 14 & 94\% \\
        & Llama-7B & 414 & 1 & 99\% \\
        
        \bottomrule
    \end{tabular}
    % \vspace{-0.1in}
    \label{tab:main_eval_go}
% \end{wraptable}
\end{table}

==> tables/models.tex <==
\begin{table*}[h]
\centering\tablesize
\caption{Model Architecture} %Change caption later
\vspace{+.15in}

\resizebox{.98\columnwidth}{!}{

\begin{tabular}{cccc}    
    % \bottomrule
    \toprule
    Model & \#Parameters & $|\vocab|$ & Finetuned \\

    \midrule
    CodeGen-350M-multi & 350M & 50400 & X \\ %need to add citation later
    WizardCoder-1B & 1B & 49153 & O \\ %Same
    Llama-7B & 6.8B & 32000 & X \\ %Same
    
    \bottomrule
\end{tabular}

}
\vspace{-0.1in}
\label{table:models}
\end{table*}

==> tables/parsers_runtime.tex <==
\begin{table}[h]
\centering
\tablesize
% \vspace{-0.32in}

\caption{Avg. time taken for a single prompt generation with LR(1) and LALR(1)}
\begin{tabular}{@{}lrrrr@{}}
    \toprule
    Model & \multicolumn{2}{c}{Python(s)} & \multicolumn{2}{c}{Go(s)} \\
    
    & LALR(1) & LR(1) & LALR(1) & LR(1) \\
    \midrule
    CodeGen-350M & 6.06 & \textbf{4.88} & 6.79 & \textbf{5.12} \\
    WizardCoder-1B & 3.00 & \textbf{1.74} & 3.69 & \textbf{1.99} \\
    \llama{} & 7.26  & \textbf{6.07} & 7.97 & \textbf{6.67} \\
    
    \bottomrule
\end{tabular}
\vspace{-0.1in}

\label{table:parsers_runtime}
\end{table}

    % CodeGen-350M & 6.06 & 6.79 & 4.88 & 5.12 \\
    % WizardCoder-1B & 3.00 & 3.69 & 1.74 &  1.99 \\
    % Llama-7B & 7.26  & 7.97  & 6.07 & 6.67 \\

% \begin{table}
% \centering
% \tablesize
% % \vspace{-0.32in}

% \caption{Avg. time taken for a single prompt generation}
% \begin{tabular}{lllll}
%     \toprule
%     Model & Language & \Baseline{}(s) & \multicolumn{2}{c}{\Tool{}(s)} \\
    
%     & & & LALR(1) & LR(1) \\
%     \midrule
%     CodeGen-350M & Python & 4.36  & 6.06 & 4.88\\
%     & Go & 4.35  & 6.79 & 5.12\\
%     \hline
%     WizardCoder-1B & Python & 1.49  & 3.00 & 1.74\\
%     & Go & 1.42  & 3.69 & 1.99\\
%     \hline
%     Llama-7B & Python & 4.88  & 7.26 & 6.07\\
%     & Go & 5.35  & 7.97 & 6.67\\
    
%     \bottomrule
% \end{tabular}
% \vspace{-0.1in}

% \label{table:runtime}
% \end{table}

==> tables/runtime.tex <==
% \begin{wraptable}{r}{.5\textwidth} \centering
% \tablesize
% \vspace{-0.32in}

% \caption{Avg. time taken for a single prompt generation}
% \begin{tabular}{lll}
%     \toprule
%     Model & \Baseline{}(s) & \Tool{}(s) \\
%     \midrule
%     CodeGen-350M & 4.36  & 9.35\\
%     WizardCoder-1B & 1.58 & 7.30\\
%     Llama-7B & 4.85 & 10.94 \\
%     \bottomrule
% \end{tabular}
% \vspace{-0.1in}

% \label{table:runtime}
% \end{wraptable}



\begin{table}
\centering
\tablesize
% \vspace{-0.32in}

\caption{Avg. time taken for a single prompt generation}
\begin{tabular}{@{}lrrrr@{}}
    \toprule
    % Model & \multicolumn{3}{c}{\Baseline{}(s)} & \multicolumn{3}{c}{\Tool{}(s)} \\
    Model & \multicolumn{2}{c}{Python(s)} & \multicolumn{2}{c}{Go(s)} \\
    
    & \Baseline{} & \Tool{} & \Baseline{} & \Tool{} \\
    \midrule
    CodeGen-350M & 4.36 & 4.88 & 4.35 & 5.12 \\
    WizardCoder-1B & 1.49 &  1.74 & 1.42 & 1.99\\
    \llama{} & 4.88 & 6.07 & 5.35 & 6.67\\
    
    \bottomrule
\end{tabular}
\vspace{-0.1in}

\label{table:runtime}
\end{table}
    %               python  go   json  python  go   json
    % CodeGen-350M & 4.36 & 4.35 & - & 4.88 & 5.12 & -\\
    % WizardCoder-1B & 1.49 & 1.42 & - & 1.74 &  1.99 & -\\
    % Llama-7B & 4.88  & 5.35  & - & 6.07 & 6.67 & -\\

% \begin{table}
% \centering
% \tablesize
% % \vspace{-0.32in}

% \caption{Avg. time taken for a single prompt generation}
% \begin{tabular}{lllll}
%     \toprule
%     Model & Language & \Baseline{}(s) & \multicolumn{2}{c}{\Tool{}(s)} \\
    
%     & & & LALR(1) & LR(1) \\
%     \midrule
%     CodeGen-350M & Python & 4.36  & 6.06 & 4.88\\
%     & Go & 4.35  & 6.79 & 5.12\\
%     \hline
%     WizardCoder-1B & Python & 1.49  & 3.00 & 1.74\\
%     & Go & 1.42  & 3.69 & 1.99\\
%     \hline
%     Llama-7B & Python & 4.88  & 7.26 & 6.07\\
%     & Go & 5.35  & 7.97 & 6.67\\
    
%     \bottomrule
% \end{tabular}
% \vspace{-0.1in}

% \label{table:runtime}
% \end{table}


